Personalised Meta-path Generation for Heterogeneous GNNs

Recently, increasing attention has been paid to heterogeneous graph representation learning (HGRL), which aims to embed rich structural and semantic information in heterogeneous information networks (HINs) into low-dimensional node representations. To date, most HGRL models rely on hand-crafted meta-paths. However, the dependency on manually-defined meta-paths requires domain knowledge, which is difficult to obtain for complex HINs. More importantly, the pre-defined or generated meta-paths of all existing HGRL methods attached to each node type or node pair cannot be personalised to each individual node. To fully unleash the power of HGRL, we present a novel framework, Personalised Meta-path based Heterogeneous Graph Neural Networks (PM-HGNN), to jointly generate meta-paths that are personalised for each individual node in a HIN and learn node representations for the target downstream task like node classification. Precisely, PM-HGNN treats the meta-path generation as a Markov Decision Process and utilises a policy network to adaptively generate a meta-path for each individual node and simultaneously learn effective node representations. The policy network is trained with deep reinforcement learning by exploiting the performance improvement on a downstream task. We further propose an extension, PM-HGNN++, to better encode relational structure and accelerate the training during the meta-path generation. Experimental results reveal that both PM-HGNN and PM-HGNN++ can significantly and consistently outperform 16 competing baselines and state-of-the-art methods in various settings of node classification. Qualitative analysis also shows that PM-HGNN++ can identify meaningful meta-paths overlooked by human knowledge.

==> pages/cover_letter.tex <==
Dear Editors:

\vspace{5mm}
We submit hereby the manuscript entitled ``Personalised Meta-path Generation for Heterogeneous Graph Neural Networks”, which we wish to be considered for publication in the journal track of the European Conference on Machine Learning and Principles and Practice of Knowledge Discovery in Databases 2022. 
No conflict of interest exists in the submission of this manuscript, 
and the manuscript is approved by all authors for publication. 
I would like to declare on behalf of my co-authors that the work described was original research that has not been published previously and is not under consideration for publication elsewhere, in whole or in part. 
All the authors listed have approved the manuscript that is enclosed.
We submit this manuscript based on the following reasons:

Heterogeneous information networks (HINs) are a ubiquitous data structure in the real world, and heterogeneous graph representation learning (HGRL) has emerged as a predominant technique for representing complex systems that are associated with multiple types of objects and relations.
However, one of the most popular HGRL paradigms is manually defining and using meta-paths to model HIN's structural and semantic information, which is still highly non-trivial.
Existing HGRL based on manual specification of meta-paths may lead to the following two limitations: 
(1) the manual meta-path design process requires prior domain knowledge, which is difficult to obtain for new complex heterogeneous information networks, and (2) nodes with the same types usually share the same predefined meta-paths, which may lead to sub-optimal representations.
Moreover, finding meaningful meta-paths from heterogeneous information networks can provide evidence for people to understand the networks better. 

To address the limitations mentioned above and motivated by the outstanding success of reinforcement learning, we propose a novel framework, Personalised Meta-path based Heterogeneous Graph Neural Network (PM-HGNN), to design task-oriented meta-paths for each node to unleash the power of HGRL.
% 
Extensive experiments conducted on different types of real-world datasets under unsupervised, semi-supervised and supervised settings exhibit the outstanding performance of PM-HGNN in network analysis tasks.
Moreover, the experiemtnal results show that PM-HGNN can discover useful meta-paths that have been ignored by human expertise.

Over the past few years, quite a lot of work tried to ameliorate the HGRL performances by better utilising meta-paths or attempting to avoid the dependency on hand-crafted meta-paths.
For instance, Hu et al. devised transferable relation scores to extract helpful structure from HIN~\cite{HDWS20}.
Yun et al. proposed GTN to select meta-paths from a group of adjacency matrices with learnable weights~\cite{YJKKK19}.
Wang et al. attempted to employ reinforcement learning technologies to discover meaningful paths between pairs of nodes for link prediction task~\cite{WDPH20}.
Nevertheless, the number of layers of~\cite{HDWS20} limits its exploration range, and also introduces a large number of additional parameters to optimise.
While \cite{YJKKK19} can only select several meta-paths for every node type, our proposed model can identify personalised meta-paths for each node.
While \cite{WDPH20} realised automatic meta-path exploration but only under link prediction tasks, we focus on the node-wise representation learning tasks in this paper. 

Regarding the appropriate reviewers for the paper, we would like to suggest researchers familiar with the HGRL because they can better understand the motivation of this work and realise its potential influence. 
For instance, Prof. Reynold C.K. Cheng, Dr Kuansan Wang, Dr Guojia Wan and Dr 	
Yuxiao Dong.


We would be very grateful if the submitted manuscript could be reviewed and considered for publication in the journal track of the European Conference on Machine Learning and Principles and Practice of Knowledge Discovery in Databases 2022. 
We thank you in advance for handling our manuscript.

% \smallskip
\vspace{4mm}
\noindent
With best regards,

\smallskip
\noindent
Yours sincerely, \\

\vspace{5mm}
\noindent
Corresponding author: \\
Name: Jun Pang \\
E-mail: \url{jun.pang@uni.lu}

==> pages/response_letter.tex <==
\section{Response Letter}
Dear Editors and Reviewers,

\smallskip
Thank you for giving us the opportunity to submit the revised draft of our manuscript titled ``Personalised Meta-path Generation for Heterogeneous Graph Neural Networks” to the journal track of the European Conference on Machine Learning and Principles and Practice of Knowledge Discovery in Databases 2022. 
We appreciate the time and efforts you have dedicated to providing valuable feedback on our manuscript. 
We are grateful to the reviewers for their insightful comments and suggestions, which helped us find our shortcomings in framework presentation, experimental evaluation, and paper writing. 
We have been able to revise the manuscript to reflect most of the suggestions provided by the reviewers. 
Below is the list of point-by-point responses to the reviewers’ comments and concerns.

\smallskip\noindent
\textbf{Comments from Reviewer 1}

\smallskip\noindent
\textbf{1.} ``1) it should be clarified what happens when a new node is added to the graph.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks for highlighting this unclear part. 
Following your suggestions, we have revised Section~\ref{subsec:model_training} and the last paragraph of Section~\ref{subsec:PM-HGNN_++} to explain the ability of PM-HGNN and PM-HGNN\textit{++} in learning representations of newly added nodes. 
Specifically, the trained reinforcement learning agent of our framework can adaptively generate a meta-path for the new node (as shown in Line $6-10$ of Algorithm~\ref{alg:PM-HGNN} and Line $5-9$ of Algorithm~\ref{alg:PM-HGNN-++}). 
After, the trained heterogeneous GNN encoder can compute node representations for the new nodes as described in Section~\ref{subsec:info_agg}.  
The learned node representations contain the information indicated by the generated meta-paths. 
}

\smallskip\noindent
\textbf{2.} ``2) a more detailed description of the experimental setting should be provided (e.g. Deep Learning / GNN framework used in the experiments).''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for the suggestion. 
We agree that the detailed description of the model configuration is essential, and we need to clarify them. 
Therefore, we describe each competing method and the implementations that we used in the experimental evaluation in Appendix~\ref{subsec:sup_competing_methods}. We have also presented the detailed model configuration in Appendix~\ref{subsec:sup_implementation_details}. 
}

\smallskip\noindent
\textbf{3.} ``Minor points:
1) better format the paper (tables and figures).
2) page 2, row 7: 'example,' $\rightarrow$ 'example;'
3) page 3, row 14: ', assume' $\rightarrow$ 'and assume'
4) page 3, rows 19-22: please, merge the two sentences 'While to learn..., we may need...'
5) page 6, row 45: should "$f: (V,E) \rightarrow R^d$" be "$f: V \rightarrow R^d$" ?
6) a general re-reading of the paper is need. There are some typos.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks for highlighting these errors. 
We have followed your suggestions to fix most of your mentioned typos. We have also carefully gone through the writing to fix other ones.
% 
The only point that we did not modify is point 5.
Heterogeneous graph representation learning based on a given heterogeneous information network $G=(V, E, N, R)$ is to integrate node attributes with relevant network structure to learn node representations.
Such a process can be more precisely depicted by $f: (V, E) \to \mathbb{R}^d$. 
}

\smallskip\noindent
\textbf{Comments from Reviewer 2}

\smallskip\noindent
\textbf{1.} ``In the problem definition, the authors should introduce the parameter that represents the maximum length of the paths. As the authors will claim in the remaining of the paper, this parameter is the one that mainly affects the time complexity of the whole algorithm.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks for pointing out this issue. 
Following your comment, we have carefully claimed the length of meta-path ($T$) in Definition 2 and have discussed how reinforcement learning generates meta-path with $T$ length in Section~\ref{subsec:solve_mdp_with_dl}. 
In the experimental parts, we empirically studied the influence of different $T$ in run time and meta-path patterns in Section~\ref{subsec:model_analysis_study}. We have also investigated different generated meta-paths with various $T$ in Section~\ref{subsec:meta-paths_analysis}. 
% 
Specifically, we find that the reinforcement learning agent can generate the same meta-paths as manually-defined ones and further explore personalised meta-paths that were ignored by expert domain knowledge. 
}

\smallskip\noindent
\textbf{2.} ``In Section 4.2, transforming different attribute spaces into the same feature space is an ambitious task that requires a strong compromise between generalization and accuracy/interpretability. The authors propose to use many encoders, but in this case, it is not possible to know what is the appropriate decoder. 
Moreover, every $W_{w_i}$ is not independent, learning each single $W_{w_i}$ requires to take into account all the other $W_{w_j}$, with $j<>i$. These aspects are not clearly discussed in the paper.
''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for the insightful comment. 
In Section~\ref{subsec:info_agg}, we propose to use node type-specific transformations to project the latent features of different node types into the same space. 
We agree that we can adopt different encoders to realise this operation, and we utilise a one-layer encoder in this paper based on empirical performance, which is given by: $H^{0}[v_{i}] = W_{\omega_{i}} \cdot x_{i}$, where $x_{i}$ and $H^{0}[v_{i}]$ are the original and projected features of node $v_{i}$, and $W_{\omega_{i}}$ is a learnable transformation matrix for the type node $\omega_{i} = \phi(v_i)$.
% 
After heterogeneous node features projection, we adopt an attention mechanism-enhanced message-passing pipeline to realise information aggregation based on adaptively generated meta-paths. 
}

\smallskip\noindent
\textbf{3.} ``Aggregation is only based on the average. This is an extreme simplification of the problem because it ignores other forms of aggregation (used in data propositionalization) and does not provide a solution for categorical attributes.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for pointing out this critical issue. 
We agree that such a shortcoming is an important issue for graphs with categorical node attributes.
In particular, we have discussed this limitation in the first paragraph of Section~\ref{subsec:PM-HGNN_++} that the definition of the state of PM-HGNN (Equation~\ref{eq:state_static}) limits the PM-HGNN's ability to distinguish the node state of categorical attributes.
% 
Moreover, we have discussed in paragraph \textbf{New State ($S$)} of Section~\ref{subsec:PM-HGNN_++} that the state definition of PM-HGNN\textit{++} can distinguish the node state with categorical attributes. 
This is mainly because PM-HGNN\textit{++} utilises the normalised node representation vector (Equation~\ref{eq:state_++}) as a node state.
$H^{t}[i]$ contains not only node attributes but also the relevant graph structure information of each node that can distinguish different nodes with categorical attributes. 
}

\smallskip\noindent
\textbf{4.} ``The results reported in Fig. 8 are not completely informative. The authors should report the actual running times, instead of a relative measure.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks for the concrete suggestion. 
Following your suggestion, we have presented the relative and actual running times of PM-HGNN and PM-HGNN\textit{++} in Figure~\ref{fig:run_time_analysis}, and have carefully gone through other figures to ameliorate the visualisation. 
From the reported meta-path generation time of the two frameworks, we can find that the longer meta-path generation process needs more run time and PM-HGNN\textit{++} requires much less run time than PM-HGNN on both datasets. 
}

\smallskip\noindent
\textbf{5.} ``The training set should be much bigger in the supervised learning setting than in the supervised learning setting.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for pointing out this important issue. 
We have explained the semi-supervised and supervised settings in Section~\ref{subsec:experimental_settings}
Particularly, the semi-supervised settings follow~[1] that utilises $400$ instances for training and another $400$ instances for validation, the rest nodes for testing.
The generated node representations are further fed into a support vector machine classifier to get the prediction results.
The train ratios that are shown in Table~\ref{tab:res_node_class} are the percentage of nodes to train the support vector machine classifier. 
Note that this setting is not the same as traditional machine learning's semi-supervised settings~[2]. 
% 
For the supervised settings, we select a group of nodes for training and employ an end-to-end mechanism to validate the effectiveness of models in different settings.
The train ratios, $15\%$ and $20\%$, adopt more nodes to train representation learning models than in semi-supervised settings. 
}

\smallskip\noindent
\textbf{6.} ``Section 4.4 information to assistant the meta-path $\rightarrow$ information to assist the meta-path''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks. 
Following your suggestion, we have fixed the typo you mentioned in Section~\ref{subsec:PM-HGNN_++} and carefully gone through the writing of the paper.
}

\smallskip\noindent
\textbf{Comments from Reviewer 3}

\smallskip\noindent
\textbf{1.} ``I would have liked to see a much deeper analysis of the meta-paths learned in the two experimental scenarios, as compared to those learned by alternative approaches and the hand-crafted ones, their ``personalized" use by different nodes and their respective utility in the downstream prediction task.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for your insightful comment. We agree that it is essential to investigate the meta-paths generated by our framework compared with other relevant approaches, i.e., hand-crafted meta-paths designed by experts and meta-paths selected from a candidate set by a certain model.
Therefore, we performed empirical studies in Section~\ref{subsec:meta-paths_analysis} to visualise how reinforcement learning agents take actions on the IMDb dataset to generate a meta-path for each node (Figure~\ref{fig:action_analysis}). 
We also summarised the statistics of PM-HGNN\textit{++}'s generated meta-paths on IMDb and compared this result with generated ones by other competing approaches. We find that the reinforcement learning agent can generate the same meta-paths as manually-defined ones and further explore new meta-paths that were ignored by expert domain knowledge. 
In addition, we mentioned in Section~\ref{sec:conclusion_and_future_work} that understanding these agent-generated meta-paths is a promising future direction to study in the context of heterogeneous graph representation learning. 
}

\smallskip
\noindent
{\bf References:}

\noindent
[1] Fu et al. MAGNN: Metapath Aggregated Graph Neural Network for Heterogeneous Graph embedding. WWW, 2020.

\noindent
[2] Kipf et al. Semi-Supervised Classification with Graph Convolutional Networks. ICLR, 2017.


==> pages/response_letter_2.tex <==
\section{Response Letter}
Dear Editors and Reviewers,

\smallskip
Thank you for giving us the opportunity to submit the revised draft of our manuscript titled ``Personalised Meta-path Generation for Heterogeneous Graph Neural Networks” to the journal track of the European Conference on Machine Learning and Principles and Practice of Knowledge Discovery in Databases 2022. 
We appreciate the time and efforts you have dedicated to providing valuable feedback on our manuscript. 
We are grateful to the reviewers for their insightful comments and suggestions, which helped us find our shortcomings in framework presentation, experimental evaluation, and paper writing. 
We have been able to revise the manuscript to reflect most of the suggestions provided by the reviewers. 
Below is the list of point-by-point responses to the reviewers’ comments and concerns.

\smallskip\noindent
\textbf{Our response to Reviewer 1:}
\textcolor{red}{
Thank you for your detailed suggestions and reviews during the first review round.
Your concerns on the description of reproducibility and discussion of inductive setting and other sections helped us polish the paper.
\\
}


\smallskip\noindent
\textbf{Comments from Reviewer 2}

\smallskip\noindent
\textbf{0.} The authors ignored most of the comments provided during my first review.

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for your time and effort in providing insightful and constructive comments on our work. We sincerely apologise for not reflecting part of your concerns in the previous revision. In the current revised manuscript, we have addressed all issues you raised and accordingly revised the manuscript.
\\
}

\smallskip\noindent
\textbf{1.} Many relational learning methods developed some years ago use the same idea exploited in this paper: use relational information to reach other instances (also of different type) and use step-by-step aggregations according to some heuristics. For instance, TILDE~\cite{BR98} learns decision trees using this approach. I could mention many of such methods that are still used. Obviously, most of them are not based on Neural Networks, but the algorithms face the same issues mentioned in the paper.
More recently, new methods for HIN node classification have been proposed. See for instance~\cite{PCKD20,SPC18,LSR20}.''

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for your detailed comments, and please accept our sincere apologies for not reflecting part of your concerns in the first revision. 
%
We have updated Section~\ref{sec:introduction} and Section~\ref{sec:related_work} to include and discuss the mentioned relevant studies on relational learning. 
For instance, in the first paragraph of Section~\ref{sec:related_work}, we gave two survey papers~\cite{V05,R08} that provide an overview of the relational learning domain.
Then, we list and discuss a series of relevant papers, i.e., ``For instance, TILDE~\cite{BR98} learns decision trees within inductive logic programming systems. 
Serafino et al.~\cite{SPC18} proposed an ensemble learning-based relational learning model for multi-type classification tasks in HINs.
Petkovic et al.~\cite{PCKD20} proposed a relational feature ranking method based on the gradient-boosted relational trees towards relational data. 
Lavrac et al.~\cite{LSR20} presented a unifying methodology combining propositionalisation and embedding techniques, which benefit from the advantages of both in solving complex relational learning tasks. 
Nevertheless, most of them are not in virtue of neural networks, which fall behind in automatically mining complex HINs.''
\\ \\
Moreover, we have further added a new state-of-the-art relational learning method~\cite{LSR20}, \textbf{PropStar}, as an additional competing model, and have reported its experimental results in Table~\ref{table:res_node_class} and Table~\ref{table:res_node_class_sup}. 
It is not surprising to find the superiority of PM-HGNN\textit{++} over \textbf{PropStar} in all datasets, due to PM-HGNN\textit{++}'s capability to generate personalised meta-paths for different nodes.
\\
}


\smallskip\noindent
\textbf{2.} What I found interesting in the paper is the wrapper-based feature extraction, where the considered meta-paths are those that provide a reward in terms of a ``downstream'' evaluation metric. This reinforcement learning approach is interesting and intriguing, but since it requires an instance-by-instance evaluation, the time complexity can be very high. Running times and time complexity analysis. 

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for the precise comments. 
We have added the discussion on the complexity analysis in Section~\ref{subsec:model_analysis}. 
Specifically, the proposed models can deal with various types of nodes and relations and fuse rich semantics in HINs. 
Benefiting from the reinforcement learning agent, personalised meta-paths are generated for different nodes, and the HGNN encoder allows information to transfer between nodes via diverse relations. 
% 
The reinforcement learning agent that we adopted in this paper, i.e., Deep Q-learning (DQN), is hard to give the precise computation complexity~\cite{FWXY20}, hence we give the empirical meta-path generation time in IMDb and DBLP datasets in Section~\ref{subsec:model_analysis_study} (Figure~\ref{fig:run_time_analysis}).
We compare the run time of PM-HGNN and PM-HGNN\textit{++} for personalised meta-paths generation.
We report their actual run time and calculate the run time of PM-HGNN\textit{++} relative to PM-HGNN (relative time on the y-axis). The results on IMDb and DBLP datasets are shown in Figure~\ref{fig:run_time_analysis}.
We can find that PM-HGNN\textit{++} is less than $5\%$ of PM-HGNN's run time on both datasets. Such results exhibit the promising time efficiency of PM-HGNN\textit{++}.
\\ \\
% 
We have added a new section to discuss the time complexity of the node representation learning process in Section~\ref{subsec:model_analysis}. 
Given a meta-path $\Omega$ and the dimensionality of (hidden) node representations is $d$. 
The time complexity of the node representation learning process is $\mathcal{O}(V_{\Omega} d^2 + E_{\Omega}d)$, where $V_{\Omega}$ is the number of nodes following the meta-path $\Omega$ and $E_{\Omega}$ is the number of meta-path based node pairs. 
$\mathcal{O}(V_{\Omega} d^2)$ accounts for the representation transformation process and $\mathcal{O}(E_{\Omega}d)$ represents the $Att(\cdot)$ computation process of relevant edges.
\\ \\
To further unfold the relationship between the complexity of generated meta-paths and the performance, we also report how the maximum step $T$ and the number of aggregation paths affect the node classification performance based on the IMDb dataset in Section~\ref{subsec:model_analysis_study} (Table~\ref{fig:max_timestep_analysis}). 
%
We can find that setting $T \geq 2$ leads to the most significant performance improvement in terms of Micro F1 over $T=1$. 
As $T$ increases, the number of aggregation paths also increases. Considering that more aggregation paths bring higher computational costs, we choose $T=2$ as the default setting in the experiments, even though $T>2$ can produce better performance.
\\
}

\smallskip\noindent
\textbf{3.} The contribution is significant, but the method, as proposed by the authors, reuses some ideas of multi-relational learning methods developed some years ago. This is not a negative aspect per se, but the problem is that the authors seem to ignore all the literature in that respect. All these methods do not use manually-defined meta paths. Comparison with state-of-the-art multi-relational learning approaches. 

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for the insightful comments and the mentioned related studies. 
We have added a discussion about relational learning approaches in Section~\ref{sec:related_work} and updated the experimental results of the state-of-the-art model, i.e., PropStar, in Section~\ref{subsec:experimental_results}.
For more details, please refer to our Response-1. 
\\ 
}

\smallskip\noindent
\textbf{4.} The experiments are performed on two (very well studied) datasets only. Additional experiments on additional datasets. 

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for the suggestion. 
We have added an additional dataset, ACM, and reported experimental results in Section~\ref{subsec:experimental_results}. 
ACM is a dataset sampled from \url{https://dl.ACM.org/}, the details on the sampling process and the data statistics are provided in Appendix~\ref{sec:appendix_datasets} and Table~\ref{table:dataset}. 
Furthermore, we have also added more analysis of the generated meta-paths on the ACM dataset in Appendix~\ref{sec:appendix_more_meta-paths_analysis}. 
\\ 
}


\smallskip\noindent
\textbf{Comments from Reviewer 3}

\smallskip\noindent
\textbf{0.} I am a bit disappointed by this revised version. While the authors agree that the questions I am raising are relevant, they seem to just restate what they already did, without reporting any further analysis. As stated in my review, I think this part is insufficient as it is now. 

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks a lot for your careful review, which are quite useful in improving our paper. We also want to sincerely apologise for not totally and concretely handling part of your concerns in the previous revision. 
In the current revised manuscript, we have carefully addressed all issues you raised and accordingly revised the manuscript. We provide the detailed settings of meta-paths across datasets and conduct a more in-depth analysis of the generated meta-paths in different datasets.
\\ \\
}


\smallskip\noindent
\textbf{1.} The specificity of the meta-paths in the IMDb case is unclear (how many other relations are there to choose from?), and this analysis was not run in the DBLP case.

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thank you for the concrete comments. We have provided more experiments and more data details to address the concerns you raised in the following four parts.
\begin{itemize}
\item First, we provide the details on all possible meta-paths for target nodes at each step of meta-path generation in Table~\ref{table:all_possible_meta_paths} for all three datasets, IMDb, DBLP, and ACM. Any of these meta-paths can be chosen as the candidate for node representation learning in HINs.
%
\item Second, we have reported the specificity of the meta-paths generated by PM-HGNN\textit{++} on IMDb dataset in Table~\ref{table:meta_paths_IMDb}. The generation of personalised meta-paths can learn to choose from all of the possible candidates listed in Table~\ref{table:all_possible_meta_paths}. In other words, when learning to generate meta-paths, any types of nodes and relations in the universal set of types can be the candidate element of meta-path.
%
\item Third, in addition to the specificity of the meta-paths on IMDb dataset, we further present those meta-paths generated by PM-HGNN\textit{++} (with different numbers of steps), Manual, and GTN~\cite{YJKKK19} on DBLP dataset in Table~\ref{table:meta_paths_DBLP}. The detailed comparison and analysis of the generated meta-paths across datasets are discussed in Section~\ref{subsec:meta-paths_analysis}. We also present how PM-HGNN\textit{++} generates different meta-paths for different target nodes on IMDb, DBLP and ACM datasets with different maximum steps in Figure~\ref{fig:action_analysis_IMDb}, Figure~\ref{fig:action_analysis_DBLP} and Figure~\ref{fig:action_analysis_ACM}, respectively. 
% \CL{(suggest to create figures like Fig.5 in DBLP and ACM datasets)}
%
\item Fourth, we have added one additional new dataset, ACM. We give the details of data statistics, all possible meta-paths, and the meta-paths generated by PM-HGNN\textit{++} in Table~\ref{table:dataset}, Table~\ref{table:all_possible_meta_paths}, and Table~\ref{table:meta_paths_ACM}, respectively. We also report the experimental results on ACM dataset in Table~\ref{table:res_node_class} and Table~\ref{table:res_node_class_sup}. Such two tables demonstrate PM-HGNN variants' superiority in the task of node classification with diverse settings.
\end{itemize}
}


\smallskip\noindent
\textbf{2.} ``I would have liked to see a much deeper analysis of the meta-paths learned in the two experimental scenarios, as compared to those learned by alternative approaches and the hand-crafted ones, their \textit{personalised} use by different nodes and their respective utility in the downstream prediction task.'' I cannot see any of these in the revised version of the manuscript.

\smallskip\noindent
\textcolor{red}{
{\it Our response:}
Thanks for your precise suggestions. 
To further understand the learned meta-paths by the proposed PM-HGNN\textit{++}, comparing to existing approaches and hand-crafted ones, we have expanded the section of Meta-path Analysis in Section~\ref{subsec:meta-paths_analysis} and Appendix~\ref{sec:appendix_more_meta-paths_analysis}. Below we summarize the revision and discussion as follows.
\begin{itemize}
\item We present how PM-HGNN\textit{++} generates different meta-paths for different target nodes on the IMDb dataset with different maximum steps in Figure~\ref{fig:action_analysis_IMDb}. 
We have also compared the meta-paths learned by PM-HGNN\textit{++} with those generated by the competing methods on IMDb data in Table~\ref{table:meta_paths_IMDb}, on DBLP data in Table~\ref{table:meta_paths_DBLP} and ACM data in Table~\ref{table:meta_paths_ACM}. 
Based on these results, we can find that the reinforcement learning agent can generate the same meta-paths as manually-defined ones and further explore new meta-paths that were ignored by expert domain knowledge. 
In addition, since PM-HGNN\textit{++} allows an available \textit{STOP} action at each step of the generation process,
PM-HGNN variants are able to produce meta-paths with flexible lengths, which cannot be fulfilled by the manually-crafted manner and GTN~\cite{YJKKK19}. 
% Due to the page limit, we added more analysis about the meta-path generated on DBLP and ACM in Appendix~\ref{sec:appendix_more_meta-paths_analysis}. 
%
\item We have also conducted an additional experiment to investigate the generated meta-paths for nodes with different classification outcomes in the last paragraph of Section~\ref{subsec:meta-paths_analysis}, i.e., Meta-path Comparison.
Specifically, this experiment aims to understand the differences of the PM-HGNN\textit{++} generated personalised meta-paths between correct and incorrect classification on nodes.
We divided nodes into two groups, \textit{pos} and \textit{neg}, according to whether applying multi-layer perceptron (MLP) with node attributes can produce correct classification under supervised settings. 
That said, correctly-classified nodes and incorrectly-classified ones are grouped into \textit{pos} and \textit{neg}, respectively.
Then, we calculate the average lengths of PM-HGNN\textit{++} generated meta-paths for nodes belonging to two groups. The results are reported in Figure~\ref{fig:meta-path_length_analysis}. 
We can find that nodes that cannot be correctly classified by MLP are associated with longer personalised meta-paths. 
Such results deliver an important insight: PM-HGNN\textit{++} tends to explore deeper relational neighbouring structures to enhance node representation learning, i.e., discriminating nodes with different labels from one another, if node attributes themselves cannot provide sufficient information. 
% 
Moreover, in the DBLP dataset, which has more complicated heterogeneous semantic patterns (4 node types and 6 relation types), node group MLP (\textit{neg}) has relatively longer meta-paths because PM-HGNN\textit{++} can have more options to explore and generate personalised meta-paths. 
\\ \\
\end{itemize}
}


% \smallskip
% \noindent
% {\bf References:}

% \noindent
% [1] H. Blockeel and L. De Raedt. Top-down induction of first-order logical decision trees. Artificial Intelligence, 101(1-2):285-297, June 1998.

% \noindent
% [2] Matej Petkovic, Michelangelo Ceci, Kristian Kersting, Saso Dzeroski: Estimating the Importance of Relational Features by Using Gradient Boosting. ISMIS 2020: 362-371

% \noindent
% [3] Francesco Serafino, Gianvito Pio, Michelangelo Ceci: Ensemble Learning for Multi-Type Classification in Heterogeneous Networks. IEEE Trans. Knowl. Data Eng. 30(12): 2326-2339 (2018)

% \noindent
% [4] Nada Lavrac, Blaz Skrlj, Marko Robnik-Sikonja: Propositionalization and embeddings: two sides of the same coin. Mach. Learn. 109(7): 1465-1507 (2020)

% \noindent
% [5] Van Otterlo, M.: A survey of reinforcement learning in relational domains. Centre for Telematics and Information Technology (CTIT) University of Twente, Tech. Rep (2005)

% \noindent
% [6] Raedt, L.D.: Logical and Relational Learning. Cognitive Technologies, (2008)

